Differential Equation Units: Learning Functional Forms of Activation Functions from Data

Most deep neural networks use simple, fixed activation functions, such as sigmoids or rectified linear units, regardless of domain or network structure. We introduce differential equation units (DEUs), an improvement to modern neural networks, which enables each neuron to learn a particular nonlinear activation function from a family of solutions to an ordinary differential equation. Specifically, each neuron may change its functional form during training based on the behavior of the other parts of the network. We show that using neurons with DEU activation functions results in a more compact network capable of achieving comparable, if not superior, performance when is compared to much larger networks.

==> compactness.tex <==
The size of a neural network is delineated its number of hidden neurons and their interconnections, which together determine the network's complexity. The ideal size of a network depends on the intricacy of the concept it is required to learn. A network that is too small cannot entirely, and circumstantially learn a hard problem.

The existing, successful structures of neural networks \cite{sutskever2014sequence, lecun2015deep, bahdanau2014neural} use hundreds of thousands to millions of parameters to learn common tasks, such as translation or object recognition. Although these tasks are complex to model, and still challenging for modern neural networks \citep{sutskever2014sequence}, they are considered "easy" when performed by a qualified human. It follows that, if we want to create a neural network with abilities that are beyond average human level aptitude, the size of such a network would need to grow considerably. For example, we have seen accuracy improvements in state-of-the-art DNNs applied to massive image classification problems resulting in part from a large increase in the number of layers \cite{he2016deep}. If this trend continues to subsist, shortly, we will witness neural networks with billions of parameters that are designed for sophisticated tasks such as live speech understanding and translation, as well as controlling robots or humanoids, which would require an immense increase in storage and computational resources.

For these reasons, we want to highlight the importance of efficient network design, and the opportunities presented by network contraction methodologies. We show that differential equation networks learn a given task with a smaller network when compared to a fixed activation DNNs. 

==> old-intro.tex <==
\eat{``Deep Learning est mort. Vive Differentiable Programming!'' -- Yann LeCun, Jan 2018.
}Driven in large part by advancements in storage, processing, and parallel computing, deep neural networks (DNNs) have become capable of outperforming other methods across a wide range of highly complex tasks. Although DNNs often produce better results than shallow methods from a performance perspective, one of the main drawbacks of DNNs in practice is computational expense. One could attribute much of the success of deep learning in recent years to cloud computing, and GPU processing. While deep learning based applications continue to be integrated into all aspects of modern life, future advancements will continue to be dependent on the ability to perform more operations, faster, and in parallel unless we make fundamental changes to the way these systems learn. 

State-of-the-art DNNs for computer vision, speech recognition, and healthcare applications require too much memory, computation, and power to be run on current mobile or wearable devices. To run such applications on mobile, or other resource-constrained devices, either we need to use these devices as terminals and rely on cloud resources to do the heavy lifting, or we have to find a way to make DNNs more compact. For example, ProjectionNet by Ravi \citep{ravi2017projectionnet}, and MobileNet by Howard et al. \citep{howard2017mobilenets} are both examples of methods that use a compact DNN representations with the goal of on-device applications. In ProjectionNet, a compact "projection" network is trained in parallel to the primary network, and used for the on-device network tasks. MobileNet proposes a streamlined architecture in order to achieve network compactness. One drawback to these approaches is that network compactness is achieved at the expense of performance. In this paper, we propose a different method for learning compact, powerful, stand-alone networks; we allow each neuron to learn its individual activation function.


Up to this point, advancements in deep learning have been largely associated with one of four areas: optimization, regularization, activation, and network structure. Some of these advancements, such as network structure, address issues related to the type of problem at hand, and the nature of the data. Since the advent of the classic feed-forward neural network (FFNN), researchers have introduced highly effective network structures such as convolutional neural networks (CNN \citep{krizhevsky2012imagenet}, popular in computer vision, and Recurrent Neural Networks (RNN) for sequences. The advent of new activation functions such as rectified linear units (ReLU) \citep{nair2010rectified}, exponential linear units (ELU) \citep{clevert2015fast}, and scaled exponential linear units (SELU) \citep{klambauer2017self} address a networks ability to effectively learn complicated functions, thereby allowing them to perform more complicated tasks. The choice of an activation function is typically determined empirically by tuning, or due to necessity. For example, in modern deep networks, the ReLU activation function is often favored over the sigmoid function, which used to be a popular choice in the earlier days of neural networks. A reason for this preference is that the ReLU function is non-saturating and does not have the vanishing gradient problem when used in deep structures \citep{hochreiter1998vanishing}. Recently, searching algorithms have proven to be valuable for automatic construction of previously hand-designed network components and activation functions \citep{zoph2017learning,bello2017neural,ramachandran2017searching}. \cite{zoph2017learning,bello2017neural,ramachandran2017searching} have proposed one such method for searching for more effective activation functions. 


\eat{Others, such as regularization, address a networks ability to generalize well when applied to new data. In addition to penalty based regularization such as L1 and L2, techniques such as dropout, drop connect, and batch normalization have been shown to produce a desirable regularization effect in deep neural networks \citep{srivastava2014dropout, wan2013regularization, ioffe2015batch}. Although modern neural networks still train using back-propagation and gradient descent, many new update rules, such as Momentum, Adagrad and RMSprop have since been introduced which contribute to the effective, and efficient learning of optimal network parameters \citep{ngiam2011optimization}. These advancements have taken deep learning to new heights, yet little effort has been dedicated to fundamentally improving the way these neural network work.}


At first glance, and from an applicability perspective, our approach is similar to max-out networks \citep{goodfellow2013maxout}, adaptive piecewise linear units by \cite{agostinelli2014learning}, and \cite{ramachandran2017searching}. However, in \cite{ramachandran2017searching}, their functions do not transform themselves during network training, and all neurons utilize the same activation function. We introduce differential equation networks (DifENs), where the activation function of each neuron is the nonlinear, possibly periodic solution of a second order, linear, ordinary differential equation. While the number of parameters learned by max-out and PLU is proportional to the number of input weights to a neuron, and the number of linear units in that neuron, for each DifEN activation function we learn only five additional parameters. 


One feature of DifENs that is particularly interesting within the healthcare industry is the ability of DifENs to regress decaying and periodic functions. Although efforts have been made to explore the usefulness of periodic functions in neural networks since the 1990s, their applicability has not yet been appreciated \citep{sopena1999neural}. Thanks to the successes of deep learning in recent years, researchers have begun re-exploring the potential of periodic functions as activations \citep{parascandolo2016taming}. This capability makes DifENs particularly well suited to problems where the desired output signals display combinations of periodicity and decay. Some examples include disease management, modeling chronic conditions such as exacerbation of COPD, medication adherence, and acute conditions that are expected to get better over time such as cancer with a successful course of treatment. Inversely, healthiness indices that might decay over time, and that could drastically effect a patients health if effectively modelled (e.g. cancer with an unsuccessful course of treatment). 


Our contributions in this paper include the following: We introduce differential equation networks, which can learn complex concepts in compact representations. We propose a learning process to learn the parameters of a differential equation for each neuron. Finally, we empirically show that a differential equation network is effective when applied to real-world problems, and that they are capable of changing activation functions during the learning process. 





==> results_old.tex <==


We have conducted several preliminary experiments using combinations
of simple functions to evaluate the performance and compactness of the
differential equation networks.


\begin{table*}[!tbh]
\caption{Networks with one hidden layer, FFNN with ReLU activations
  (1) vs. DifEN (2). The second and third columns report the number of
neurons in the hidden layer.}
\label{comp-table}
\centering
\begin{tabular}{lllllllll}
  \toprule
  Data Set  & Size 1 & Size 2   & Acc 1 & Acc 2 & AUC 1 & AUC 2 & F1 1
  & F1 2  \\
  \midrule
  IONOSPHERE & 10 & 4 & 0.8826 & \bf{0.9061} & 0.8819 & \bf{0.9154} & 0.8779  & \bf{0.9047}  \\
  FOURCLASS & 10 & 4 & 0.6705 & \bf{0.7187} & 0.5563 & \bf{0.7132} & 0.5383  & \bf{0.6909}  \\
  DIABETES & 10 & 2 & 0.7554 & \bf{0.7662} & 0.8035 & \bf{0.8094} & 0.7519  & \bf{0.7631}  \\
  A1A & 10 & 2 & 0.8436 & \bf{0.8450} & 0.8938 & \bf{0.8996} & 0.8406
                                                                       & \bf{0.8448}\\
\bottomrule
\normalsize
\end{tabular}
\label{table_uci}
\end{table*}

\subsection{Toy Regression Datasets}

We ran several tests on toy regression problems. We compared a 
ReLU network to a
significantly smaller DifEN. The datasets consisted of two toy function
approximation problems. We chose a simple sine function ($y(t) =
\sin(t)$) and a more complex function involving oscillation and
periodic decay  ($y(t)=\frac{\sin(3t) - \cos ^2 (4t) } {2} +
\frac{4(\cos^{-1}(\sin(t/4)) + 1)}{3}$). The DifEN consistently
outperforms larger ReLU networks as shown in
figures~\ref{fig:sin_1period} and \ref{fig:sin_1period_cust}. We fully
tuned the ReLU network and found that a  ReLU network ten times
larger than its DifEN counterpart the DifEN still won in performance (two
hidden layers in each, 100 and 50, vs. 10 and 5 for ReLU and DifEN respectively).  

\subsection{UCI Datasets}
We compared a small DifEN to a larger ReLU
FFNN on a few standard benchmark datasets. We ran three trials for
each dataset and averaged the results. On average, the small DifEN showed a $3\%$ accuracy gain over its considerably larger ReLU counterpart. 
We did not regularize either network; performance would likely
be improved by imposing regularization such as L2 penalty, dropout and
batch normalization. Results are
summarized in Table~\ref{table_uci}.




\eat{
\begin{figure*}[!tbh]
\centering  
\subfigure[ ]{\includegraphics[width=0.21\linewidth]{../charts/sin_approx_tf_2period_100neurons_1layer.pdf}}\label{fig:sin_approx_tf_2period_100neurons_1layer}
\subfigure[ ]{\includegraphics[width=0.21\linewidth]{../charts/sin_approx_tf_2period_100neurons_2layer.pdf}}\label{fig:sin_approx_tf_2period_100neurons_2layer}
\subfigure[ ]{\includegraphics[width=0.21\linewidth]{../charts/sin_approx_tf_2period_20ReLU_1layer.pdf}}\label{fig:sin_approx_tf_2period_100neurons_2layer}
\subfigure[
]{\includegraphics[width=0.21\linewidth]{../charts/sin_approx_diffeqnet_2period_3neurons_1layer.pdf}}\label{fig:sin_approx_diffeqnet_2period_3neurons_1layer}
\subfigure[ ]{\includegraphics[width=0.21\linewidth]{../charts/custom_sigmoid_100_50_1.pdf}}\label{fig:sin_approx_tf_2period_100neurons_2layer}
\subfigure[ ]{\includegraphics[width=0.21\linewidth]{../charts/custom_relu_100_50_1.pdf}}\label{fig:sin_approx_tf_2period_100neurons_2layer}
\subfigure[ ]{\includegraphics[width=0.21\linewidth]{../charts/custom_fcn_10_5_1_x.pdf}}\label{fig:sin_approx_diffeqnet_2period_3neurons_1layer}
\subfigure[ ]{\includegraphics[width=0.21\linewidth]{../charts/custom_relu_10_5_1.pdf}}\label{fig:sin_approx_diffeqnet_2period_3neurons_1layer}
\caption{Top: Learning to regress the toy function
  $y(t)=\frac{sin(2t) + 1}{2}$.  (a) Fixed activation FFNN approximation with 1 hidden layer
  comprising 100 sigmoid neurons $(MSE=0.0276)$. (b) Fixed activation FFNN
  approximation with 2 hidden layers, each comprising 100 sigmoid neurons (200
  total) $(MSE<4e^{-5})$. (c) Fixed activation FFNN
  approximation with 1 hidden layers, each comprising 20 ReLU neurons $(MSE=0.00768)$. (d) The differential equations network
  achives near perfect function approximation with one hidden layer
  comprising 2 neurons. The neurons are initialized with ReQU and ReLU
  ($a=1,
  b=0,c=0$ and $a=0,
  b=1,c=0$ respectively) $(MSE<1e^{-6})$.\\
Bottom: Learning to regress the toy function
  $y(t)=\frac{\sin(3t) - \cos ^2 (4t) } {2} + \frac{4(\cos^{-1}(\sin(t/4)) + 1)}{3}$. FFNN with two hidden layers (100 in the first and 50 neurons in
  the second layer) fixed neurons in one hidden layer: (e) sigmoids
  ($MSE = 0.﻿0932$) (f)
  ReLUs ($MSE = 0.﻿0632$)  (g) DifEN with a 10 times smaller network (two hidden layers, 10 in the first and 5 neurons in
  the second layer)
  with randomly initialized differential equations.  ($MSE = 0.﻿0155$) 
  (h) FFNN with a 10 times smaller network (two hidden layers, 10 in the first and 5 neurons in
  the second layer)
  withReLU activations.  ($MSE = 0.1151$) 
}
 \label{fig:sin_1period}
\end{figure*}

}


\subsection{MNIST}
We will compared performance of a simple, single hidden layer FFNN
equipped with DifEN neurons, to that of a network of the same size,
but with one of several standard activation function. We did not use
any of the usual DNN bells and whistles for this experiment
(e.g. dropout). We tested the assumptions that the DifEN should
outperform the others with the same archetecture, or at least match
performance with a smaller number of neurons. We ran 3 fold cross
validation and report the mean result for each activation. We tracked
performance changes as we increased the size of the single hidden
layer. DifENs have more hyperparameters that can influence the
performance of the network. For example, we optimized weights and
coefficients using different learning rates, and found it benificial to update them according to different strategies. We updated the weights at every minibatch, but the coefficients were updated only once per epoch.

\begin{figure}[!tbh]
\centering  
\includegraphics[width=1.0\linewidth]{../charts/mnist_accuracy_by_network_size_full2.pdf}
\caption{MNIST classification accuracy by network size. Size here represents the number of neurons in each network's single hidden layer.}
\label{fig:mnist_acc_comp}
\end{figure}


\begin{table}[!tbh]
\caption{Comparison of performance on MNIST by network size and activation}
\centering
\begin{tabular}{llllll}
  \toprule
  Activation & 10n & 20n & 40n & 60n & 100n \\
  \midrule

  ReLU & .9217 & .9328 & .9503 & .9576 & .9683 \\
  SELU & .9207 & .9422 & .9588 & .9684 & .9730 \\
  ELU & .9218 & .9413 & .9530 & .9619 & .9705 \\
  LReLU & .9262 & .9429 & .9533 & .9643 & .9712 \\
  DifEN & \bf{.9307} & \bf{.9489} & \bf{.9650} &  \bf{.9718} & \bf{.9742} \\

\bottomrule
\normalsize
\end{tabular}
\label{table_mnist}
\end{table}



\subsection{CIFAR10}
For this experiment we compared two version of ResNet18, one standard
\cite{he2016deep}, and one with a single DifEN layer preceding the
final fully connected layer. The smaller architecture was chosen to
measure the effect of a single DifEN layer on performance, not to
achieve the state-of-the-art results, which would require many more layers.

\eat{
\begin{figure}[!tbh]
\centering  
\includegraphics[width=0.47\linewidth]{../charts/cifar10_training_curve_comp.pdf}
\caption{CIFAR10 training error by version. V1 shows the output from ResNet18 unchanged and V2 shows the training curve for ResNet18 modified with a single layer if DifEN directly preceding the final fully connected layer}
\label{fig:cifar10_training_comp}
\end{figure}
}

\begin{table}[!tbh]
\caption{Comparison of performance on CIFAR10 - V1 is a standard version of ResNet18 while V2 inserts a single DifEN layer (of the same size) directly before the final fully connected layer}
\centering
\begin{tabular}{lll}
  \toprule
  Data Set & Version & Accuracy \\
  \midrule
  CIFAR10 & V1 & 0.8554 \\
          & V2 & \bf{0.8601} \\
\bottomrule
\normalsize
\end{tabular}
\label{table_vision}
\end{table}



\subsection{Discussion}
We have shown that DifEN activation functions transform during the training process (e.g. change from sigmoid to ReLU). 
We have also demonstrated the capability of DifENs to learning complex concepts will, and with a significantly reduced network size. Table \ref{table_mnist} shows a DifEN with 60 neurons can out perform much larger network utilizing ReLU, LReLU and ELU activations with 100 neurons. Moreover, Fig. \ref{fig:sin_approx_diffeqnet_2period_3neurons_1layer} shows DifENs have the capability to learn a better approximation when compared to a network with ReLU activations throughout. The ability of DifENs to achive top-notch performance with a compact representation makes them a good candidate for on-device applications. In addition to on-device applications, DifENs seem well suited to applications that that require the capabilities of a large neural network, but are currently limited by memore, or latency issues associated with sending information back and forth for heavy processing such as space applications and robotics. 



\begin{figure}[!tbh]
\centering  
\subfigure[ ]{\includegraphics[width=0.47\linewidth]{../charts/sin_approx_tf_2period_100neurons_1layer.pdf}}\label{fig:sin_approx_tf_2period_100neurons_1layer}
\subfigure[ ]{\includegraphics[width=0.47\linewidth]{../charts/sin_approx_tf_2period_100neurons_2layer.pdf}}\label{fig:sin_approx_tf_2period_100neurons_2layer}
\subfigure[ ]{\includegraphics[width=0.47\linewidth]{../charts/sin_approx_tf_2period_20ReLU_1layer.pdf}}\label{fig:sin_approx_tf_2period_100neurons_2layer}
\subfigure[
]{\includegraphics[width=0.47\linewidth]{../charts/sin_approx_diffeqnet_2period_3neurons_1layer.pdf}}\label{fig:sin_approx_diffeqnet_2period_3neurons_1layer}
\caption{Learning to regress the toy function
  $y(t)=\frac{sin(2t) + 1}{2}$.  (a) Fixed activation FFNN approximation with 1 hidden layer
  comprising 100 sigmoid neurons $(MSE=0.0276)$. (b) Fixed activation FFNN
  approximation with 2 hidden layers, each comprising 100 sigmoid neurons (200
  total) $(MSE<4e^{-5})$. (c) Fixed activation FFNN
  approximation with 1 hidden layers, each comprising 20 ReLU neurons $(MSE=0.00768)$. (d) The differential equations network
  achives near perfect function approximation with one hidden layer
  comprising 2 neurons. The neurons are initialized with ReQU and ReLU
  ($a=1,
  b=0,c=0$ and $a=0,
  b=1,c=0$ respectively) $(MSE<1e^{-6})$.
}
 \label{fig:sin_1period}
\end{figure}




\begin{figure*}[!tbh]
\subfigure[ ]{\includegraphics[width=0.24\linewidth]{../charts/custom_sigmoid_100_50_1.pdf}}\label{fig:sigmoid_approx_complex}
\subfigure[ ]{\includegraphics[width=0.24\linewidth]{../charts/custom_relu_100_50_1.pdf}}\label{fig:relu_approx_complex}
\subfigure[ ]{\includegraphics[width=0.24\linewidth]{../charts/custom_fcn_10_5_1_x.pdf}}\label{fig:sin_approx_diffeqnet_2period_3neurons_1layer}
\subfigure[ ]{\includegraphics[width=0.24\linewidth]{../charts/custom_relu_10_5_1.pdf}}\label{fig:sin_approx_diffeqnet_2period_3neurons_1layer}
\caption{
\eat{
Top: Learning to regress the toy function
  $y(t)=\frac{sin(2t) + 1}{2}$.  (a) Fixed activation FFNN approximation with 1 hidden layer
  comprising 100 sigmoid neurons $(MSE=0.0276)$. (b) Fixed activation FFNN
  approximation with 2 hidden layers, each comprising 100 sigmoid neurons (200
  total) $(MSE<4e^{-5})$. (c) Fixed activation FFNN
  approximation with 1 hidden layers, each comprising 20 ReLU neurons $(MSE=0.00768)$. (d) The differential equations network
  achives near perfect function approximation with one hidden layer
  comprising 2 neurons. The neurons are initialized with ReQU and ReLU
  ($a=1,
  b=0,c=0$ and $a=0,
  b=1,c=0$ respectively) $(MSE<1e^{-6})$.\\
Bottom: 
}
Learning to regress the toy function
  $y(t)=\frac{\sin(3t) - \cos ^2 (4t) } {2} + \frac{4(\cos^{-1}(\sin(t/4)) + 1)}{3}$. FFNN with two hidden layers (100 in the first and 50 neurons in
  the second layer) fixed neurons in one hidden layer: (a) sigmoids
  ($MSE = 0.﻿0932$) (b)
  ReLUs ($MSE = 0.﻿0632$)  (c) DifEN with a 10 times smaller network (two hidden layers, 10 in the first and 5 neurons in
  the second layer)
  with randomly initialized differential equations.  ($MSE = 0.﻿0155$) 
  (d) FFNN with a 10 times smaller network (two hidden layers, 10 in the first and 5 neurons in
  the second layer)
  withReLU activations.  ($MSE = 0.1151$) 
}
 \label{fig:sin_1period_cust}
\end{figure*}


